Neural-Symbolic Inference for Robust Autoregressive Graph Parsing via Compositional Uncertainty Quantification

Pre-trained seq2seq models excel at graph semantic parsing with rich annotated data, but generalize worse to out-of-distribution (OOD) and long-tail examples. In comparison, symbolic parsers under-perform on population-level metrics, but exhibit unique strength in OOD and tail generalization. In this work, we study compositionality-aware approach to neural-symbolic inference informed by model confidence, performing fine-grained neural-symbolic reasoning at subgraph level (i.e., nodes and edges) and precisely targeting subgraph components with high uncertainty in the neural parser. As a result, the method combines the distinct strength of the neural and symbolic approaches in capturing different aspects of the graph prediction, leading to well-rounded generalization performance both across domains and in the tail. We empirically investigate the approach in the English Resource Grammar (ERG) parsing problem on a diverse suite of standard in-domain and seven OOD corpora. Our approach leads to 35.26% and 35.60% error reduction in aggregated Smatch score over neural and symbolic approaches respectively, and 14% absolute accuracy gain in key tail linguistic categories over the neural model, outperforming prior state-of-art methods that do not account for compositionality or uncertainty.

==> algorithm/algorithm.tex <==
\begin{algorithm*}[ht]
\caption{Neural-symbolic Inference}\label{alg:neural-symbolic-inference}
% \small
\textbf{Input:} $\langle \mathcal{L}, \mathcal{G} \rangle = \{\langle L_1, G_1\rangle, ...,  \langle L_K, G_K\rangle\}$  is the group of all predictions for one sentence, where $K$ is the beam size.\\
The top $k^\text{th}$ prediction is $\langle L_k, G_k\rangle$, where $L_k = \langle S_k, P_k\rangle$ is the linearization ($S_k$ is the sequence of tokens and $P_k$ is the token-level beam score), and $G_k = \langle N_k, E_k \rangle$ is the corresponding graph ($N_k$ is the node set and $E_k$ is the edge set).\\
$G_0$ is the ACE graph, $p_0$ is the weight set for ACE.\\
\textbf{Output:} Optimal $G_*$ from meta graph $G_{\text{Meta}*}$
\begin{algorithmic}[1]
\State $\langle \mathcal{L}_\Delta, \mathcal{G}_\Delta \rangle = \textsc{LCS\_cluster}(\langle \mathcal{L}, \mathcal{G} \rangle)$ \Comment{Graph clustering based on the longest common string (LCS)}
\State $\text{score}_* \gets 0, G_{\text{Meta}*} \gets \langle \emptyset, \emptyset \rangle$
\For{$\langle \mathcal{L}_\delta, \mathcal{G}_\delta \rangle \in \langle \mathcal{L}_\Delta, \mathcal{G}_\Delta \rangle$}
    \State $\mathcal{G}_{p\delta} = \textsc{AssignProb}(\mathcal{G}_\delta, P_\delta)$ \Comment{Assign probabilities to the nodes and edges in the graph}
    \State $G_{\text{Meta}} = \textsc{GraphMerge}(\mathcal{G}_{p\delta})$ \Comment{Merge the graphs in the cluster into the candidate meta graph}
    \State $\text{score} = \textsc{Smatch}(G_{\text{Meta}}, G_0)$
    \If{$\text{score} \geq \text{score}_*$}
        \State{$\text{score}_* \gets \text{score}, G_{\text{Meta}*} \gets \textsc{GraphMerge}(G_{\text{Meta}}, G_0)$}
        % \State $G_{\text{Meta}*} \gets \textsc{GraphMerge}(G_{\text{Meta}}, G_0)$ \Comment{Merge ACE graph to the meta graph}
    \EndIf
\EndFor
\State $G_\text{Final} \gets \textsc{Pruning}(G_{\text{Meta}*}), G_* \gets \langle \emptyset, \emptyset \rangle$ \Comment{Construction inference: pruning subgraphs}
% \State $G_* \gets \langle \emptyset, \emptyset \rangle$
\For{$N/E \in G_\text{Final}$} \Comment{Node/Edge inference}
    \State $R_* \gets 0, n_*/e_* \gets NULL$
    \For{$\langle n/e, p\rangle \in N$}
        \State $\alpha = \sigma(\frac{1}{T}(\log(p)+B)), R = \alpha * p + (1-\alpha) * G_0.\textsc{Exists}(n/e) * p_0$
        \If{$R \geq R_*$}
        \State{$R_* \gets R$, $n_*/e_* \gets n/e$}
        \EndIf
    \EndFor
    \State $G_*.\textsc{Add}(n_*/e_*)$
\EndFor\\
\Return{$G_*$} 
\end{algorithmic}
\end{algorithm*}
